Regularising orientation estimation in Cryo-EM 3D map refinement through measure-based lifting over Riemannian manifolds

Motivated by the trade-off between noise-robustness and data-consistency for joint 3D map reconstruction and rotation estimation in single particle cryogenic-electron microscopy (Cryo-EM), we propose ellipsoidal support lifting (ESL), a measure-based lifting scheme for regularising and approximating the global minimiser of a smooth function over a Riemannian manifold. Under a uniqueness assumption on the minimiser we show several theoretical results, in particular well-posedness of the method and an error bound due to the induced bias with respect to the global minimiser. Additionally, we use the developed theory to integrate the measure-based lifting scheme into an alternating update method for joint homogeneous 3D map reconstruction and rotation estimation, where typically tens of thousands of manifold-valued minimisation problems have to be solved and where regularisation is necessary because of the high noise levels in the data. The joint recovery method is used to test both the theoretical predictions and algorithmic performance through numerical experiments with Cryo-EM data. In particular, the induced bias due to the regularising effect of ESL empirically estimates better rotations, i.e., rotations closer to the ground truth, than global optimisation would.

==> sections/4-cryo-em.tex <==
\section{Single particle Cryo-EM}
\label{sec:cryo-prelim}
This section provides a brief overview of the inverse problem in single particle Cryo-EM. 
We start out by briefly describing the application area (\cref{sec:cryo-em}) and then shift focus to formulating the inverse problem mathematically (\cref{sec:maths-of-cryo-em}).
Emphasis here is on the case with homogeneous particles, which corresponds to joint 3D reconstruction and rotation estimation.
The discussion is then centered around solving the joint recovery problem. 
That is, we discuss and review existing mathematical results and algorithms and consider the problem of noise-robustness versus data-consistency in performing joint recovery in this context 
(\cref{sec:lifting-orientation-related-work}).

\subsection{Cryo-EM in structural biology}
\label{sec:cryo-em}
Biological macromolecules (or biomolecules), like proteins and nucleic acids, are critical in biological processes that sustain both life and disease. 
Their structure (3D `shape') along with its dynamics plays a key role in understanding their function in specific biochemical reactions.
Much attention has therefore been devoted to methods for determining such structures and their dynamics and much of structural biology focuses on this.

Historically, protein structures are computationally determined from X-ray crystallography data.
This involves solving a challenging inverse problem and both experimental and algorithmic progress in the field has been extremely successful, thus turning X-ray crystallography into a standard method in structural biology for structure recovery of biomolecules.
However, an inherit drawback with X-ray crystallography is that the approach is by design restricted to studying structures of biomolecules in crystalline state, thus making it difficult to uncover conformational dynamics. 
The technique is also not possible to use on biomolecules, such as membrane proteins, that are difficult, if not impossible, to crystallise.
In contrast, cryogenic electron microscopy (Cryo-EM) opens up for the possibility to study biomolecules in their native aqueous environment. 
The field has made rapid advances in the last few years regarding both sample preparation, instrumentation and computational methods. This development was recognised through the 2017 Nobel Prize in Chemistry.

Single particle Cryo-EM is a specific Cryo-EM technique that uses principles from tomography to computationally determine the 3D structure of a biomolecule and potentially also uncover the multiple states representing its dynamics.
The starting point is to prepare an aqueous solution that contains a large number of copies of the biomolecule to be studied, where each copy is referred to as a \emph{particle}.
Next, cryofixation is applied to this solution, resulting in a thin slab of vitrified ice that contains these particles.
The slab is then imaged in a high-resolution transmission electron microscope (TEM) resulting in several 2D phase contrast images (micrographs).
Next, image processing techniques are used to extract several 2D image patches from each micrograph. Each such patch represents a noisy 2D \enquote{projection image} of a \emph{single} particle in an unknown pose, the latter encoding its 3D rotation and 2D in-plane translation w.r.t.\@ a common 3D reference.
The aim is now to computationally recover a volumetric representation of the 3D structure of the biomolecule (3D map) from these aforementioned 2D image patches.

It is clearly not possible to independently recover a 3D map of each particle from the corresponding single 2D image patch that is a \enquote{projection image} of the former. 
Therefore, a key assumption in single particle Cryo-EM is that \emph{all} particles are copies of the \emph{same biomolecule}.
This assumption is then used in mathematical techniques from tomography to recover a 3D map of the biomolecule from the aforementioned 2D image patches.
An important case is when the biomolecule is rigid (homogeneous particles).
Then, all particles can be assumed to have (approximately) identical 3D maps and the 2D image patches represent tomographic data of a single 3D object. 
In that setting, once particle specific poses are determined, it is possible to use standard mathematical techniques from tomography to recover the 3D map from the 2D image patches.
A more challenging case is when the biomolecule is flexible (heterogeneous particles). The goal is now to recover a dynamical 3D map from the 2D image patches, which is significantly more challenging.

Finally, a recovered 3D map is a volumetric representation of the 3D electrostatic potential generated by the biomolecule and the surrounding aqueous buffer. This 3D map can in principle be used to determine the exact location of each atom in the biomolecule, i.e., its 3D atomic model  \cite{Nakane:2020aa,Bouvier:2020aa}.
% This is currently a semi-automatic process that requires a large degree of human intervention, and it is only feasible when the 3D map has high enough resolution (at least 0.2~nm, preferably around 0.1~nm).
% Currently, such a resolution is only reachable for biomolecules that are sufficiently rigid (no dynamics). 



% and [rewrite] revisits an open problem in joint 3D map reconstruction and rotation estimation in single particle Cryo-EM

% [mention that we will discuss the cryo-em imaging pipeline and revisit rotation estimating to argue how lifting will resolve issues here]

% \subsection{Revisiting rotation estimation in Cryo-EM}
% As already stated, the aim in single particle Cryo-EM is in the homogeneous setting to recover the 3D map. The unknown particle specific  rotations act as nuisance parameters, which either need to be estimated or averaged out. 

% \todo[inline]{Continue stitching stuff back together after rewrite ozan. @JAN: Do not review this section yet}

% A natural mathematical question is whether formal uniqueness holds for the joint problem of recovering the 3D map and estimating the rotations. Such an analysis is performed assuming data is noise-free. In a simplistic setting where the model for TEM imaging (forward operator) is given by a parallel beam ray transform, one can, except for some special cases, prove formal uniqueness up to a global orthogonal transformation \cite{lamberg2008unique}. Interestingly, adopting a more realistic TEM imaging model (based on Born approximation and TEM optics) allows one to prove uniqueness without any global orthogonal transformation \cite{Kurlberg:2021aa}.

% On the algorithmic side, common approaches in single particle Cryo-EM are based on variational models. In that context, the variant of \cref{eq:model-problem} that corresponds to rotation estimation is not the full problem. Solving it is, however, one of the central challenges so much effort has been devoted this in the Cryo-EM community.

% In the following, we provide a brief survey of this development. Note that these methods tend to utilise additional special structure of the objective in \cref{eq:model-problem} and the fact that $\manifold=\mathrm{SO}(3)$. As such, they stand in contrast to research on manifold optimisation pursued within the mathematical community, which focuses on methods for solving general optimisation problems on manifolds with provable convergence guarantees.

% Early approaches were not based on any variational models, instead they relied on integral geometry. As such, these approaches model TEM imaging with the parallel beam ray transform. In this setting, a key observation  was that one can estimate rotations without having access to a 3D map. Indeed, as suggested as early as 1986 \cite{Vainshtein1986}, through common lines of the 2D projections in Fourier space relative rotations can be retrieved. Soon after that the method of moments \cite{goncharov1987methods,goncharov1988integral,goncharov1988determination,salzman1990method} was proposed and later further improved and analyzed \cite{basu2000feasibility,basu2000uniqueness}, which did not need any information on the 3D map either.
% % observation [is common lines] suggested in 1986 \cite{Vainshtein1986} and soon after the method of moments \cite{goncharov1987methods}\cite{goncharov1988integral}\cite{goncharov1988determination}\cite{salzman1990method}.] [both did not need any information on what the protein looked like, but would have enough information from the images]
% In practice, the high noise levels in Cryo-EM data were the first major hurdle for these methods. Already, the method of moments breaks down under these high noise conditions, and it has shown to be difficult to make the method more noise-robust. The common lines method on the other hand -- although also breaking down under high noise in the standard form -- has had several extensions that have turned out to be more noise-robust than the original method \cite{bandeira2020non,shkolnisky2012viewing,singer2010detecting,singer2011three,wang2013rotation}.
% % has been difficult to work around
% % espite theoretical underpinnings of moments \cite{basu2000feasibility} \cite{basu2000uniqueness} the latter method broke down under high noise conditions, which was difficult to work around] 


% % [rotation estimation has undergone several paradigms in Cryo-EM]
% % [- people believed that it was necessary to get the rotations before 3D map reconstruction [ab initio and refinement]]
% % [- people believed that one should really work around getting rotations [ab init and in refinement]]




% % very old works - split into common lines and moments
% % lines
% % \cite{Vainshtein1986} % [1986] Determination of the spatial rotation of arbitrarily arranged identical particles of unknown structure from their projections

% % moments
% % \cite{goncharov1987methods} % [1987] Methods of integral geometry and finding the relative rotation of identical particles arbitrarily arranged in a plane from their projections onto a straight line
% % \cite{goncharov1988integral} % [1988] Integral geometry and three-dimensional reconstruction of randomly oriented identical particles from their electron microphotos
% % \cite{goncharov1988determination} % [1988] Determination of mutual rotation of identical particles from their projections by the moments method
% % \cite{salzman1990method} % [1990] A method of general moments for orienting 2D projections of unknown 3D objects

% % [The common line method has had several extensions that have turned out to be more noise-robust than the original method]
% % % ab initio
% % \cite{singer2010detecting} % [2010] Detecting consistent common lines in cryo-EM by voting
% % % % all the work here that actually recovers an rotation
% % \cite{bandeira2020non,shkolnisky2012viewing,singer2011three,wang2013rotation} % [go here a bit more into detail what people cooked up to do rotation estimation with]

% There have also been other approaches that attempted to cope with the noise through working around direct estimation of the rotations. A -- by now famous -- example in Cryo-EM is Kam's auto-correlation analysis, which dates back to 1980 \cite{kam1980reconstruction}. Similarly to the common lines approach several, Kam's method has been inspiration for several extensions \cite{bhamre2015orthogonal,levin20183d,sharon2020method} and methods in the same spirit \cite{bandeira2017estimation}. 
% % autocorrelation
% % \cite{kam1980reconstruction} % [1980] The reconstruction of structure from electron micrographs of randomly oriented particles
% % [but after that several [more recently] other methods in the same or slightly different spirit have been proposed]
% % % work that does not actually recover the rotations
% % \cite{bandeira2017estimation,bhamre2015orthogonal,levin20183d,sharon2020method}

% Recently, also deep learning-based methods for rotation estimation have been proposed \cite{banjac2021learning}. However, these methods work without explicit considerations of the high noise levels and results are not competitive with the model-based approaches yet.
% % [And even more recently, also deep learning based approaches have been explored]
% % learning rotations
% % \cite{banjac2021learning} % [2021] Learning to recover rotations from projections in single-particle cryo-EM

% % % 3D map reconstruction focussed contributions
% % \cite{gordon1970algebraic} % [1970] Algebraic reconstruction techniques (ART) for three-dimensional electron microscopy and X-ray photography
% % \cite{radermacher2007weighted} % [2007] Weighted back-projection methods

% % \cite{abrishami2015fast} % [2015] A fast iterative convolution weighting approach for gridding-based direct Fourier three-dimensional reconstruction with correction for the contrast transfer function 
% % \cite{barnett2017rapid} % [2017] Rapid solution of the cryo-EM reconstruction problem by frequency marching
% % \cite{donati2018fast} % [2018] Fast multiscale reconstruction for cryo-EM
% % \cite{donati2019inner} % [2019] Inner-loop-free admm for cryo-em
% % \cite{li2014wavelet} % [2014] Wavelet frame based algorithm for 3D reconstruction in electron microscopy
% % % sub - deep learning
% % \cite{kimanius2020exploiting} % [2020] Exploiting prior knowledge about biological macromolecules in cryo-EM structure determination

% Apart from noise, a second hurdle is structural heterogeneity of particles. That is, the assumption that all particles are the same does not hold true in practice. For this reason and other factors such as improper alignment of the 2D projection images, there is typically some refinement stage after the \textit{ab initio} phase as described above. The current paradigm is still to work with explicit rotations, but approaches have evolved over time.

% % [From the early days of

% % The paradigm has been the same since the early days. That is iterative schemes with alternating 3D map and rotation updates]


% % [However, in real-world data, where there is also structural heterogeneity, which has to be accounted for [...]]
% % [when people wanted higher resolution 3D maps ...]
% % [The paradigm has been the same since the early days. That is iterative schemes with alternating 3D map and rotation updates]

% Early work on iterative refinement can be traced back as early as 1972 \cite{gilbert1972iterative} and to follow up works such as \cite{harauz1983direct}, where typically a 3D map update step alternated with an rotation alignment step. These type of algorithms were also the cornerstone of the first generation of software packages \cite{frank1996spider,ludtke1999eman,van1996new} and most software packages being released in the years after followed this approach \cite{grigorieff2007frealign,hohn2007sparx,shaikh2008spider,sorzano2004xmipp,tang2007eman2}.
% % optimisation through refinement
% % early work
% % \cite{gilbert1972iterative} % [1972] Iterative methods for the three-dimensional reconstruction of an object from projections
% % \cite{harauz1983direct} % [1983] Direct three-dimensional reconstruction for macromolecular complexes from electron micrographs

% % [These typically alternated between analytic
% % methods in Fourier space for the 3D map reconstruction and rotation alignment]
% % software early
% % \cite{frank1996spider} % [1996] SPIDER and WEB: processing and visualization of images in 3D electron microscopy and related fields
% % \cite{ludtke1999eman} % [1999] EMAN: semiautomated software for high-resolution single-particle reconstructions
% % Software later
% % \cite{van1996new} % [1996] A new generation of the IMAGIC image processing system

% % [Most software packages being released in the years after followed this approach] \cite{grigorieff2007frealign} \cite{hohn2007sparx} \cite{shaikh2008spider}\cite{sorzano2004xmipp}\cite{tang2007eman2}
% % \cite{sorzano2004xmipp} % [2004] XMIPP: a new generation of an open-source image processing package for electron microscopy
% % \cite{grigorieff2007frealign} % [2007] FREALIGN: high-resolution refinement of single particle structures
% % \cite{hohn2007sparx} % [2007] SPARX, a new environment for Cryo-EM image processing
% % \cite{tang2007eman2} % [2007] EMAN2: an extensible image processing suite for electron microscopy
% % \cite{shaikh2008spider} % [2008] SPIDER image processing for single-particle reconstruction of biological macromolecules from electron micrographs


% Arguably, starting from the 2010 there has been a shift in rotation estimation in refinement, and there are now two packages dominating the field: RELION \cite{scheres2012relion} and cryoSPARC \cite{punjani2017cryosparc}. Rather than picking one rotation after every alignment step -- which can suffer from high noise levels -- RELION gives probabilities to each rotation and marginalizes over a large set. Although technically solving a different problem now, this method tends to be very robust to noise because of this averaging approach. CryoSPARC on the other hand uses a branch-and-bound algorithm for the rotation estimation, which is more sophisticated than plain alignment, faster than the RELION approach (and solves the original problem), but arguably pays in noise-robustness.
% % \cite{scheres2012relion} % [2012] RELION: implementation of a Bayesian approach to cryo-EM structure determination
% % \cite{de2016scipion} % [2016] Scipion: A software framework toward integration, reproducibility and validation in 3D electron microscopy
% % \cite{reboul2018rapid} % [2018] Rapid near-atomic resolution single-particle 3D reconstruction with SIMPLE
% % \cite{punjani2017cryosparc}


% Even more recently, deep learning-based methods have been introduced to joint refinement. Here too approaches differ whether to work around the rotations through marginalisation \cite{gupta2021cryogan} or whether to try to actually find them through a multi-scale solver \cite{zhong2021cryodrgn2}.
% % % heterogeneity
% % \cite{gupta2021cryogan} % [2021] CryoGAN: a new reconstruction paradigm for single-particle cryo-EM via deep adversarial learning [[working around estimating rotations is also prevalent in deep learning approaches for refinement]]
% % [or whether to try to actually find it]
% % \cite{zhong2021cryodrgn2} % [2021]

% In any case the refinement methods proposed so far, either model-based or learning-based, do not really use the manifold structure of $\mathrm{SO}(3)$ as well as they could -- unlike the \textit{ab initio} methods -- and in works where this is attempted \cite{zehni2020joint}, the authors resort to local charts, which have the drawbacks as denoted above. Potentially there is plenty to be won here.
% % misc
% % \cite{zehni2020joint} % [2020] Joint Angular Refinement and Reconstruction for Single-Particle Cryo-EM
% % [Potentially, there is a lot to be won here.]


% % \todo[inline]{maybe also mention that people viewed rotation estimation as something that was more of a nuisance parameter}



% % \begin{itemize}
% %     \item rotation estimation in Cryo-EM
% %     \begin{itemize}
% %         \item Ab initio + limitations
% %         \item Joint refinement
% %         \begin{itemize}
% %             \item Historical papers towards the main paradigms we have now
% %             \item In the end we see a trade-off between numerical stability (RELION) and high-accuracy (Cryo-Sparc)
% %         \end{itemize}
% %     \end{itemize}
%     % \item Manifold-valued optimisation
%     % \begin{itemize}
%     %     \item Optimisation on manifolds
%     %     \begin{itemize}
%     %         \item Papers 90s + Absil book smooth
%     %         \item Typically these methods can guarantee local convergence (and not necessarily to a global minimiser) [also put previous paper here]
%     %         \item Often even works if objective function is non-smooth]
%     %     \end{itemize}
%     %     \item Global optimisation typically on Hadamard manifolds (where we have convexity)
%     %     \begin{itemize}
%     %         \item Again smoothness is not really an issue
%     %         \item In the case of special structure there are numerous efficient algorithms papers Ronny
%     %     \end{itemize}
%     %     \item For global minimisation on general manifolds there are several limitations for suitable methods for Cryo-Em
%     %     \begin{itemize}
%     %         \item Comes down to computational feasibility: eg particle based methods (stochastic or deteministic) have the drawback that many particles are needed
%     %         \item as the algorithm typically needs to be done multiple times, this can become too expensive
%     %     \end{itemize}
%     %     \item Lifting can overcome this, but there haven't been any theoretical guarantees so far
%     %     \item So here lies a mathematical and practical question we aim to address in this work
%     % \end{itemize}
% % \end{itemize}

% % [should actually focus on global optimisation here (mention that on hadamard spaces we have a myriad of optimisation methods - On non-hadamard spaces we have either local convergence [eg, my old paper] or global convergence under KL constraints, but not to a global minimiser)]


% \begin{itemize}
%     \item Notation
%     \begin{itemize}
%         \item 3D map, data, spaces, forward operator etc.
%     \end{itemize}
% \end{itemize}

% \todo{Check feedback Ozan in first year report about this part}



% \paragraph{The Cryo-EM forward operator}
% An extensive overview on TEM image formation is provided in \cite{oktem2015mathematics}, we will mainly follow \cite{zickert2020analytic}.

% In Cryo-EM we are interested in the 3D structure of a particle, which is given by a scalar field $\vol \colon \Real^3 \to \Real$ representing the 3D electrostatic potential (\emph{3D map}) generated by the particle embedded in vitrified aqueous buffer. An example of such a 3D map is shown in \cref{fig:clean70SRibosome-vol}.
% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=0.4\linewidth]{"images/clean70SRibosome_vol.png"}
%     \caption{Surface rendering of a 3D map representing the electrostatic potential of a 70S ribosomal subunit.}
%     \label{fig:clean70SRibosome-vol}
% \end{figure}
% It is not possible to directly observe the 3D map. Instead, the particle embedded in vitrified aqueous buffer is imaged in a TEM. This results in a noisy 2D phase contrast image of the 3D map.

% The relation between the 3D map and this 2D image is given by a model for the TEM image formation. 
% Mathematically, it can be modeled by a mapping $\forward \colon \volSpace \to \imgSpace$ (\emph{forward operator}) that maps a 3D map $\vol \colon \Real^3 \to \Real$, which is an element in a Hilbert space $\volSpace$, into an image $\img \colon \Real^2 \to \Real$, which is an element in the Hilbert space $\imgSpace$. The weak-phase object approximation \cite{vulovic2014use} allows us to express $\forward$ as a parallel beam ray transform along the TEM optical axis (tomographic projection) followed by a 2D convolution in the detector plane to account for TEM optics and detector response, see \cite{oktem2015mathematics} for the details:
% \begin{equation}
%     \forward(\vol) := \RerCTF \ast \bigl(\projection(\vol)\bigr).
%     \label{eq:cryo-operator}
% \end{equation}
% The convolution in \cref{eq:cryo-operator} is a 2D convolution in the detector plane. The convolution kernel $\RerCTF \colon \imgSpace \to \imgSpace$ is given analytically by its Fourier transform:
% \begin{equation}
%     \ReCTF(\xi) := - \biggl(\sqrt{1 - \ampContrast^2} A(\xi) \sin\Bigl(\frac{\defocus}{2 k}|\xi|^{2}-\frac{\spAberration}{4 k^{3}}|\xi|^{4} \Bigr) 
%     + \alpha A(\xi) \cos\Bigl(\frac{\defocus}{2 k}|\xi|^{2}-\frac{\spAberration}{4 k^{3}}|\xi|^{4}	\Bigr)
%     \biggr).
%     \label{eq:ctf}
% \end{equation}
% In the above, $\defocus$ is the \emph{defocus depth}, $\spAberration$ is the \emph{spherical aberration constant}, $\waveNumber$ is the \emph{wave number} of the imaging electron, and $\ampContrast$ is the \emph{amplitude contrast ratio}. Next, $A$ is the aperture function, which is an indicator function on a disc with a radius that is determined by the TEM objective aperture. Finally, $\projection \colon \volSpace \to \imgSpace$ is the `projection mapping'. Choosing a coordinate system where the $\eC$-axis is parallel to the TEM optical axis allows us to express the projection mapping as
% \begin{equation}
%     \projection \vol (\eA,\eB) := \int_{-\infty}^\infty \vol(\eA,\eB,\eC) \mathrm{d} \eC.
% \end{equation}


% \paragraph{The inverse problem in single particle Cryo-EM}
% For the case with homogeneous particles, one can mathematically express the inverse problem in single particle Cryo-EM as the task of recovering a 3D map $\vol \in \volSpace$ from 2D projection images $\img_1, \ldots, \img_\numImgs \in \imgSpace$. Here, each $\img_{\imgInd} \in \imgSpace$ is a single sample of the $\imgSpace$–valued random variable $\stimg_{\imgInd}$ such that 
% \begin{equation}
%     \stimg_\imgInd = \forward(\rot_\imgInd . \vol) + \stnoise_\imgInd 
%     \quad\text{with $\rot_\imgInd\in \mathrm{SO}(3)$ and $\stnoise_{\imgInd} \sim \PDDataNoise^{\imgInd}$ for $\imgInd=1,\ldots, \numImgs$}
% \end{equation}
% where $\rot.\vol := \vol \circ \rot^{-1}$ for $\rot\in \mathrm{SO}(3)$ and $\PDDataNoise^{\imgInd}$ is the distribution of the $\imgSpace$-valued random variable $\stnoise_\imgInd$ representing the observation noise.
% Note here that the 3D rotations $\rot_\imgInd\in \mathrm{SO}(3)$ of the $\imgInd$:th particle that generated the image $\img_{\imgInd}$ are unknown.


% it is key that these images are taken under different projection angles. However, the TEM electron beam only has limited angular range. To overcome this, not just one frozen particle is considered, but tens of thousands of particles are imaged. Since these particles are frozen under different rotations, the limited angle problem is overcome. The downside to this method is that there might be some structural heterogeneity in the particles as many macro-molecules such as proteins are inherently flexible and have moving parts. In this work structural homogeneity  will be assumed, i.e., the images are generated from rotations of a ground truth 3D map. Including a noise model, the observations can be modeled as noisy projections of a rotated particle, i.e.,
% \begin{equation}
%     \img_\imgInd = \forward \rot_\imgInd . \vol + \stnoise_\imgInd \quad\text{with $\rot_\imgInd\in \mathrm{SO}(3)$ and $\stnoise_{\imgInd} \sim \PDDataNoise^{\imgInd}$ for $\imgInd=1,\ldots, \numImgs$},
% \end{equation}
% where $\rot.\vol := \vol \circ \rot^{-1}$ for $\rot\in \mathrm{SO}(3)$. In other words, the inverse problem amounts not only to retrieving the 3D map $\vol$, but also to estimating an rotation $\rot_\imgInd$ for every image $\img_\imgInd$.

\subsection{Survey of reconstruction methods for single particle Cryo-EM}
\label{sec:lifting-orientation-related-work}
% State-of-the-art approaches for jointly recovering the 3D map and estimating 3D particle rotations in single particle Cryo-EM are based on a variational model of the form
% \begin{align}
% \label{eq:unlifted-problem-cryo-vol-rot-abstract-spaces}
%     \inf_{\substack{\vol \in \volSpace \\ \rot_1, \ldots, \rot_\numImgs \in \mathrm{SO}(3)}} \biggl\{ \sum_{\imgInd=1}^\numImgs \Bigl[ \frac{1}{2\noiseLevelParam_{\imgInd}} 
%     \bigl\|
%       \forward (\rot_{\imgInd}.\vol)-\img_{\imgInd}
%     \bigr\|_\imgSpace^{2} \Bigr] 
%     + \regA(\vol) \biggr\}.
% \end{align}
% Here, $\noiseLevelParam_{\imgInd}>0$ is a weight that depends on the data noise level and $\regA \colon \volSpace\to\Real$ is a suitably chosen convex regularisation functional. 

% Note that if particle specific 3D rotations $\rot_\imgInd$ were known, recovering the 3D map amounts to convex minimisation, which can be pursued using standard techniques from optimisation.
% In contrast, if the 3D map $\vol$ is known, estimating particle specific 3D rotations rotations $\rot_\imgInd$ requires one to solve a non-convex minimisation problem. 
% The non-convexity  is due to the non-linear structure of the underlying manifold $\mathrm{SO}(3)$ and properly handling it is very difficult, if not impossible, when data is highly noisy, which is typically the case with Cryo-EM data. 
% % \begin{remark}
% % The problem in \cref{eq:unlifted-problem-cryo-vol-rot-abstract-spaces} is not the most general case even particles are assumed to be homogeneous. In practice, the underlying biomolecule might have certain rotational symmetries \cite{jiang2017atomic} given by some group $\rotsSubGroup\subset\mathrm{SO}(3)$. Furthermore, the 2D TEM images might not be properly aligned, i.e., there is some additionally in-plane translation $t_\imgInd\in \Real^2$ for each image. From an optimisation point of view the former causes ill-posedness because of non-uniqueness and the latter makes an already non-convex problem higher dimensional and thus more challenging. The ill-posedness can be resolved by optimising over the submanifold $\mathrm{SO}(3)/\rotsSubGroup$ and in the case of in-plane shifts the optimisation will be over the $\bigl( \mathrm{SO}(3)/\rotsSubGroup \bigr)\times \Real^2$ manifold. 
% % % This work aims to provide an algorithm that can be extended to this more general case, i.e., it should work for general Riemannian manifolds by design.
% % \end{remark}
% % We next provide a brief survey of mathematical and algorithmic work related to reconstruction in single particle Cryo-EM.
% % As already stated, the aim in single particle Cryo-EM is in the homogeneous setting to recover the 3D map. The unknown particle specific  rotations act as nuisance parameters.
% % , which either need to be estimated or averaged out. 


